Deriving Quests from Open World Mechanics

Open world games present players with more freedom than games with linear progression structures. However, without clearly-defined objectives, they often leave players without a sense of purpose. Most of the time, quests and objectives are hand-authored and overlaid atop an open world's mechanics. But what if they could be generated organically from the gameplay itself? The goal of our project was to develop a model of the mechanics in Minecraft that could be used to determine the ideal placement of objectives in an open world setting. We formalized the game logic of Minecraft in terms of logical rules that can be manipulated in two ways: they may be executed to generate graphs representative of the player experience when playing an open world game with little developer direction; and they may be statically analyzed to determine dependency orderings, feedback loops, and bottlenecks. These analyses may then be used to place achievements on gameplay actions algorithmically.

==> approach.tex <==
beforehand. 


==> workscited.tex <==
While these algorithms are useful for determining the optimal places for progression in theory, it remains to be seen if these locations are as ideal in practice. The theories presented are based solely on rules derived from Minecraft and it remains to be seen if they can be applied to other games with similar effectiveness. There is also the issue of testing said effectiveness. User studies comparing the two methods would provide valuable insight into what factors make a particular type of objective more engaging. Minecraft already had an achievement system in place which allowed us to confirm our results, however it will be necessary to test if these patterns emerge in games without progression systems.
